Turkish MMLU Pro: Traceable Option Augmentation and Its Validity Limits in Turkish Multiple-Choice Evaluation

Adding answer options can lower multiple-choice scores without improving assessment validity. Turkish MMLU Pro examines this distinction using 12,000 Turkish-source questions across 58 sections. Each question retains its stem, five original options and source key, and receives five options copied from other questions in the same section. Sentence-embedding retrieval proposes candidates; a language model selects existing identifiers. Deterministic verification reconstructs all 60,000 additions. A 25-model calibration exposes scoring and generation-budget effects. Five evaluations produce source-key accuracies of 34.8%-81.4%. On 981 shared questions, one API-served model falls from 93.7% with five choices to 83.1% with ten; 102 of 115 lost correct responses select borrowed options. The decrease is 24.4 percentage points on heuristically flagged negative stems and 5.9 points elsewhere. A completed human-checked audit of 200 sampled questions, with undocumented reviewer tool use, yields 47 and 31 multiple-answer judgments across the two record sets, 25 of the latter unresolved. These records support concern about ambiguity, while their dependence and incomplete reviewer-method documentation limit validation. Because order and labels also change, the paired comparison measures augmentation as implemented. The contribution is a traceable construction and an analysis of its validity limits, not evidence that lower ten-choice scores measure knowledge better.

==> tables/borrowed_choice.tex <==
\code{gemma4:31b-mlx} & 4,345 & 2,696 & 62.0 & [60.6, 63.5]\\
\code{gemma4:26b-mlx}$^{\dagger}$ & 5,076 & 3,135 & 61.8 & [60.4, 63.1]\\
\code{gemma4:e4b-mlx} & 6,663 & 3,893 & 58.4 & [57.2, 59.6]\\
\code{qwen3.5:4b-mlx} & 7,799 & 4,428 & 56.8 & [55.7, 57.9]\\
\code{gpt-6-astra} & 2,223 & 1,577 & 70.9 & [69.0, 72.8]\\


==> tables/cross_benchmark.tex <==
\code{gpt-6-astra} & -- & 81.4 & 93.3$^{\S}$ & -- & --\\
\code{muse-glimmer:30b-mlx} & 32.3 & 65.0$^{*}$ & 84.9 & -- & --\\
\code{gemma4:31b-mlx} & 31.7 & 63.6 & 84.4$^{\ddagger}$ & 85.2 & 88.4\\
\code{qwen3.8:27b-mlx} & 27.8 & 63.0$^{*}$ & 80.8 & -- & --\\
\code{qwen3.6:27b-mlx} & 27.8 & 60.0$^{*}$ & 80.0 & -- & --\\
\code{qwen3.5:27b-mlx} & 27.4 & 58.0$^{*}$ & 82.9$^{\ddagger}$ & 86.1 & --\\
\code{gemma4:26b-mlx}$^{\dagger}$ & 26.2 & 57.5 & 80.2 & 82.6 & 86.3\\
\code{qwen3.5:35b-mlx} & 35.1 & 57.0$^{*}$ & 80.1$^{\ddagger}$ & 85.3 & --\\
\code{gemma4:12b-mlx} & 12.4 & 55.0$^{*}$ & 72.7 & 77.2 & 83.4\\
\code{qwen3.5:9b-mlx} & 9.4 & 48.0$^{*}$ & 73.6$^{\ddagger}$ & 82.5 & --\\
\code{gemma4:e4b-mlx} & 8.1 & 44.4 & -- & 69.4 & 76.6\\
\code{granite4.2:30b} & 29.3 & 42.0$^{*}$ & -- & 77.6 & --\\
\code{qwen3.5:4b-mlx} & 4.5 & 34.8 & 68.2$^{\ddagger}$ & 79.1 & --\\
\code{granite4.2:8b} & 8.8 & 31.0$^{*}$ & -- & 74.0 & --\\
\code{nemotron-3.5-lightning:30b-mlx} & 32.9 & 31.0$^{*}$ & 59.8 & 81.9 & --\\
\code{gemma4:e2b-mlx} & 5.2 & 30.0$^{*}$ & -- & 60.0 & 67.4\\
\code{qwen3.5:2b-mlx} & 2.2 & 16.0$^{*}$ & 56.2$^{\ddagger}$ & 55.3 & --\\
\code{granite4.2:3b} & 3.7 & 13.0$^{*}$ & -- & 67.8 & --\\
\code{qwen3.5:0.8b-mlx} & 0.9 & 13.0$^{*}$ & 45.2$^{\ddagger}$ & 29.7 & --\\


==> tables/exclusions.tex <==
conflicting answer keys & 12,120 \\
duplicate choices & 414 \\
duplicate question stems & 32,696 \\
option dependent choice & 976 \\
possible missing visual & 133 \\


==> tables/full_run.tex <==
\multicolumn{11}{@{}l}{\emph{Open-weight models, run locally}}\\
\code{gemma4:31b} & 31.7 & nvfp4 & 63.64 & [62.78, 64.50] & 99.85 & 18/0 & 0 & 1.1/258 & 11.56 & 63 [53, 72]\\
\code{gemma4:26b}$^{\dagger}$ & 26.2 & nvfp4 & 57.51 & [56.62, 58.39] & 99.81 & 23/0 & 0 & 1.1/260 & 1.98 & 60 [50, 69]\\
\code{gemma4:e4b} & 8.1 & nvfp4 & 44.42 & [43.53, 45.31] & 99.94 & 7/0 & 0 & 1.0/1 & 1.13 & 42 [33, 52]\\
\code{qwen3.5:4b} & 4.5 & nvfp4 & 34.84 & [33.99, 35.70] & 99.83 & 20/1 & 0 & 1.2/2,048 & 1.68 & 40 [31, 50]\\
\midrule
\multicolumn{11}{@{}l}{\emph{API-served models}}\\
\code{gpt-6-astra} & -- & API & 81.38 & [80.68, 82.07] & 99.91 & 11/0 & 5,529 & 27.7/790 & 0.81$^{\ddagger}$ & --\\


==> tables/option_lengths.tex <==
Original & 60,000 & 24.08 & 16 & 71 \\
Added & 60,000 & 18.13 & 13 & 51 \\


==> tables/preview_sections.tex <==
AUZEF & 207 \\
Adalet & 206 \\
Aşçılık & 207 \\
Bankacılık ve Sigortacılık & 207 \\
Büro Yönetimi ve Yönetici Asistanlığı & 207 \\
DHBT & 207 \\
Dini Bilgiler & 207 \\
Dış Ticaret & 206 \\
Ehliyet & 207 \\
Elektrik Enerjisi Üretim,İletim ve Dağıtımı & 207 \\
Emlak ve Emlak Yönetimi & 207 \\
Ev İdaresi & 207 \\
Felsefe & 207 \\
Fotoğrafçılık ve Kameramanlık & 207 \\
Futbol & 207 \\
Halkla İlişkiler ve Reklamcılık & 206 \\
Halkla İlişkiler ve Tanıtım & 207 \\
KPSS & 206 \\
KPSS Denemeleri & 207 \\
Kamu Yönetimi & 207 \\
Kim 500 Milyar İster & 207 \\
Kültürel Miras ve Turizm & 207 \\
Laborant ve Veteriner Sağlık & 207 \\
Lojistik & 207 \\
Marka İletişimi & 207 \\
Medya ve İletişim & 207 \\
Menkul Kıymetler ve Sermaye Piyasası & 207 \\
Muhasebe ve Vergi Uygulamaları & 207 \\
Parakende Satış ve Mağaza Yöneticiliği & 207 \\
Radyo ve Televizyon Programcılığı & 207 \\
Sağlık Kurumları İşletmeciliği & 207 \\
Sağlık Yönetimi & 207 \\
Siyer & 207 \\
Sosyal Hizmet & 207 \\
Sosyal Hizmetler & 207 \\
Sosyoloji & 207 \\
Spor Yönetimi & 207 \\
TUS & 207 \\
Tarih & 207 \\
Tarım & 207 \\
Turizm ve Otel İşletmeciliği & 206 \\
Turizm ve Seyehat Hizmetleri & 207 \\
Türk Dili ve Edebiyatı & 207 \\
Tıbbi Dökümantasyon ve Sekreterlik & 207 \\
Uluslar Arası İlişkiler & 207 \\
Uluslararası Ticaret ve Lojistik Yönetimi & 207 \\
YGS Denemeleri & 207 \\
Yaşlı Bakımı & 206 \\
Yerel Yönetimler & 207 \\
Yönetim Bİlişim Sistemleri & 207 \\
Çalışma Ekonomisi ve Endüstri İlişkileri & 207 \\
Çağrı Merkezi Hizmetleri & 207 \\
Çocuk Gelişimi & 207 \\
Özel Koruma ve Güvenlik & 207 \\
İktisat & 207 \\
İlahiyat & 207 \\
İnsan Kaynakları Yönetimi & 207 \\
İşletme Yönetimi & 207 \\

